Magnification of Photometric LRGs by Foreground LRGs and Clusters in SDSS

The magnification effect of gravitational lensing is a powerful probe of the distribution of matter in the universe, yet it is frequently overlooked due to the fact that its signal to noise is smaller than that of lensing shear. Because its systematic errors are quite different from those of shear, magnification is nevertheless an important approach with which to study the distribution of large scale structure. We present lensing mass profiles of spectroscopic luminous red galaxies (LRGs) and galaxy clusters determined through measurements of the weak lensing magnification of photometric LRGs in their background. We measure the change in detected galaxy counts as well as the increased average galaxy flux behind the lenses. In addition, we examine the average change in source color due to extinction by dust in the lenses. By simultaneously fitting these three probes we constrain the mass profiles and dust-to-mass ratios of the lenses in six bins of lens richness. For each richness bin we fit an NFW halo mass, brightest cluster galaxy (BCG) mass, second halo term, and dust-to-mass ratio. The resulting mass-richness relation is consistent with previous analyses of the catalogs, and limits on the dust-to-mass ratio in the lenses are in agreement with expectations. We explore the effects of including the (low signal-to-noise) flux magnification and reddening measurements in the analysis compared to using only the counts magnification data; the additional probes significantly improve the agreement between our measured mass-richness relation and previous results.

==> response <==
** Abstract
- the authors should define alpha_c,m

We removed the reference to the alphas in the abstract, as it is a minor point and adding the definition would be cumbersome.

- the abstract states that flux magnification has low S/N but the authors conclude that better constraints come from flux magnification than number counts. It should be clarified in the abstract

We claim that better constraints come from combining flux magnification with number counts, not that flux magnification provides better constraints than number counts (the opposite is true).  We've added more information in the paper (see below) such that is more clear.


** Introduction
- 3rd para.: "traditionally ... with shear" and "its statistical errors": I would compare S/N's instead of errors alone. Shear has a very low S/N due to the ellipticity dispersion (~1/30). Magnification bias noise is mainly proportional to Poisson error, which makes higher S/N measurement with fewer galaxies than shear

We've added more detail to the signal-to-noise comparison.  The actual comparison depends on the alpha values.  We've added an example to be more concrete on the issue:
"The signal-to-noise of the magnification of source galaxies behind a lens is typically smaller than that of the galaxies' shear 
(see Schneider et al. 2000, equ. 7).  The exact ratio depends on the shape of the lens mass profile and the sources' lensing sensitivity $\alpha_{c}$, 
defined below in equation 15, but for a singular isothermal sphere lens and a given number of sources with the same $\alpha_{c}$ as in this work, 
the signal-to-noise of the magnification effect is about a factor of three smaller than that of lensing shear."


- 4th para.: "different lensing probe", more precisely, magnification measures the convergence of lensing in the weak lensing regime.
- 5th para.: Coupon et al. (2013) measured the change in distribution of spectroscopic redshifts.
- 6th para.: "a signal qualitatively similar to, and much stronger than" : this statement is only partly true: whereas physical correlation is expected to be positive, magnification can range from negative to positive, and the physical correlation signal strength depends on the contamination rate. I see what the authors want to say, but in the regime explored here only a positive magnification signal is expected and the contamination may be high due to the use of nearby background sources with photo-z's. In the studies cited right after, some measured a negative magnification signal from very deep observations. Could you please rephrase this?
- the paper by Umetsu et al. (2012) is missing from the citations I think.

** Sec. 2
-Is the weak lensing approximation really justified? It wouldn't change the conclusions of the paper so it can remains as it is, however the authors should write later that it is used for Eqs. 10 and 13 and write the equation delta_mu ~ 2 X kappa.

** Sec. 2.1
- I don't quite understand the demonstration for alpha_m. The authors need to better explain the derivation of Eq. 9, in particular to emphasise the difference with the "C_s" term as described in Ménard et al. (2010), Eq. (A4). Is it possible to show the dN/dM for the LRG sample? I find the variation of alpha_m quite large between 19.0 and 19.9 and I wonder why it becomes so large (-0.20) approaching the limiting magnitude of ~ 20.0. I would expect that the distribution of galaxies would be closer to a power low compared to the QSO distribution used in Ménard et al. (2010) and be therefore much smaller than the value of 0.35 they find.

** Sec. 2.2
- The two first equations have no numbers.
- Please explicitly write how Eq. (11) is built from the two previous ones.

** Sec. 3
- The authors should probably give more details here, in particular they need to better explain what is the difference between the extinction A_V and the opacity of the dust K_ext.
- Does the dust-to-mass ratio gamma change with respect to galaxy type and redshift ?

** Sec. 4
- It might be helpful to remind that "i" refers to i-band.

** Sec. 4.3
- What is the order of magnitude for the dust correction?

** Sec 5.1.1
- Halo miscentering especially affects small scales, it would be useful to have a quantified estimate of the minimum scale the effect starts to hit given the S/N of this study.
- Halo miscentering also affects convergence and shear differently. Please make sure it is taken into account.

** Sec 6.1
- last sentence: do the authors claim that the uncertainties on alpha_c from intrinsic correlations are properly measured from the jackknife resampling? Can they give justification on this?

** Sec. 6.2.2
- Do all LRGs lenses have spectroscopic redshifts?

** Sec. 7
- Is the modelled signal stacked as well ? Or only the mean value of the richness bins is fitted? Since the mass-richness slope becomes very steep for massive haloes, taking the mean will bias the value measured from stacks in the more massive richness bins (see Eq. 15 of Ford et al 2012). Note: I think it goes the other way around as the systematic offset seen in Fig. 11 for the most massive bins, but it might be worth checking it anyway.

** Sec 8
- since photo-z codes can fit extinction values, it would be easy to confirm the upper limits found for the extinctions values. It is however well known that elliptical galaxies at low redshift have low extinction values. Alternatively, the authors may cite values from the literature for elliptical galaxies (i.e. other than Ménard et al.'s).
- As written above, it would be interesting to have a quantitative estimate of dust corrections on alpha's.
- About the figures (not compulsory but recommended):
        - it would be more helpful to compare the different richness bins for one observable than to compare different observables for one richness bin (the current format). In addition the authors could gain space by sticking plots to each other and increase the size to gain in readability.
        - another suggestion: the increase in lensing signal is not as clear as the authors state given the current plot configuration. It could be presented differently, for example with one plot as function of richness using only one integrated value (say up to 0.1 degree) per richness bin.

** Sec. 8.1
- I think it would interesting to show the magnitude shift results independently in Fig. 11 (or in appendix if the authors really want to keep the figure as is); I worry that given the lower statistical significance of other probes compared to number counts, their signal would be much lower than that of number counts.

** Sec. 8.2
- It is probably not surprising to find a low reddening for LRG, the comparison with Ménard et al. at sec. 9 might be moved to this section

** Sec. 8.4.2
- the tests on contamination is interesting but not sufficient. The authors seem to neglect the possible higher contamination in clusters where the density of galaxies is also higher. In addition their source sample of LRG resembles that of cluster members at low redshift, which will further increase the probability to find outlier associated with clusters. Here is a  few solutions to improve the credibility of their results:
      - the authors could estimate the ratio of LRG with spectro-z around cluster positions and redshift < 0.4, compared to the rate of outliers in general with z < 0.4 (and possibly show the result in Fig. 1),
      - or the authors could use simulations (populating haloes or directly take semi-analytic catalog - do the authors have access to the MICE simulations?) by randomly picking 1.2% of galaxies and compute the relative contribution of galaxies inside clusters and in the field,
      - compute magnification for the total sample and cut into several redshift bins (make sure to understand completeness issues),
      - or use BOSS QSO's to confirm their measurements.

** Sec. 9
- Because the contamination rate is probably higher in cluster environment, I don't agree with the statement the contribution from overlap is well understood and insignificant (see above points).
